Izhikevich-Inspired Temporal Dynamics for Enhancing Privacy, Efficiency, and Transferability in Spiking Neural Networks

Biological neurons exhibit diverse temporal spike patterns, which are believed to support efficient, robust, and adaptive neural information processing. While models such as Izhikevich can replicate a wide range of these firing dynamics, their complexity poses challenges for directly integrating them into scalable spiking neural networks (SNN) training pipelines. In this work, we propose two probabilistically driven, input-level temporal spike transformations: Poisson-Burst and Delayed-Burst that introduce biologically inspired temporal variability directly into standard Leaky Integrate-and-Fire (LIF) neurons. This enables scalable training and systematic evaluation of how spike timing dynamics affect privacy, generalization, and learning performance. Poisson-Burst modulates burst occurrence based on input intensity, while Delayed-Burst encodes input strength through burst onset timing. Through extensive experiments across multiple benchmarks, we demonstrate that Poisson-Burst maintains competitive accuracy and lower resource overhead while exhibiting enhanced privacy robustness against membership inference attacks, whereas Delayed-Burst provides stronger privacy protection at a modest accuracy trade-off. These findings highlight the potential of biologically grounded temporal spike dynamics in improving the privacy, generalization and biological plausibility of neuromorphic learning systems.

==> sections/Summary.tex <==
% \section{Summary}
\noindent
We developed two biologically inspired spike generation mechanisms to model diverse temporal firing patterns observed in real neurons: Poisson-burst and Delayed-burst dynamics. The Poisson-Burst mechanism models neuronal activity by generating bursts of spikes at regular time intervals, where the likelihood of a burst occurring is proportional to the input intensity. When a burst is triggered, the number of spikes it contains is sampled from a Poisson distribution, introducing stochastic variability across bursts. This approach mimics the behavior of cortical neurons that fire in temporally clustered patterns, with the occurrence of bursts reflecting stimulus-driven modulation.
% The Poisson-burst mechanism captures the variability in spike count by generating bursts of spikes whose size follows a Poisson distribution, with burst frequency modulated by input intensity—mimicking cortical neurons that fire in temporally clustered bursts. 
The Delayed-burst mechanism generates a single burst per input, where the timing of the burst is sampled from a Geometric distribution, inversely related to input strength – capturing dynamics observed in sensory neurons that convey stimulus intensity through spike timing. Together, these mechanisms leverage distinct statistical distributions to model different temporal response patterns in spiking systems, enabling systematic exploration of how spike-timing and spike-count variability influence predictive performance and privacy in neural networks. An illustration of these two dynamics is shown in Figure~\ref{fig:enc}.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=1\linewidth, height=0.45\linewidth]{Figure/SNNEncoders.pdf}
    % \includegraphics[width=\linewidth]{Figure/mia_1sm.png}
    \caption{Illustration of two biologically inspired temporal spike dynamics. (\textbf{Left}) \textit{Poisson-Burst} generates bursts with spike counts sampled from a Poisson distribution, modeling input-dependent repetitive firing. (\textbf{Right}) \textit{Delayed-Burst} introduces latency-based onset, where stronger inputs trigger earlier fixed-size bursts. Rows represent increasing input intensity from top to bottom.}
    \label{fig:enc}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=.8\linewidth, height=0.35\linewidth]{Figure/MIA_updated.pdf}
    % \includegraphics[width=\linewidth]{Figure/mia_1sm.png}
    \caption{Membership Inference Attack (MIA) Framework}
    \label{fig:mia_24}
\end{figure}




% This study explores how biologically inspired temporal spike dynamics affect model utility, privacy leakage, system efficiency, and transferability in spiking neural networks (SNNs). While modern SNNs typically rely on Leaky Integrate-and-Fire (LIF) neurons for scalability, these simplified units overlook the diverse firing patterns observed in biological neurons. Inspired by the Izhikevich model, which captures dynamics such as bursting and latency-based spiking, we investigate whether similar temporal features can be introduced through input-level spike encoding rather than neuron-level changes.

% We implement four spike transformation schemes: Burst, Poisson-Burst, Delayed-Burst, and Delayed-Poisson. These vary in burst size and onset timing, emulating patterns found in cortical and sensory neurons. Each encoding converts normalized inputs into spike trains over $T = 100$ timesteps, preserving compatibility with standard LIF-based architectures. We evaluate these spike dynamics across four dimensions: model performance, privacy vulnerability, system efficiency, and transferability.



Membership Inference Attacks (MIA) are used to quantify privacy leakage. An attacker’s goal is to infer whether a given input was used to train a target model. To simulate this, we adopt a shadow model approach: the shadow model, architecturally identical to the target, is trained on a disjoint 80\% split of the dataset. It is then queried on both its training and test sets, with the outputs labeled as ‘IN’ and ‘OUT’ respectively to reflect membership status. These labeled outputs are used to train a binary SVM attack model. Finally, the attack model is evaluated on the target model’s outputs—using samples drawn from both the target’s training and test sets—to determine whether each sample was part of the training distribution. Membrane potentials from the final timestep serve as input features, and Area Under the ROC Curve (AUC) is used to measure attack success where lower AUC implies stronger privacy. The overall pipeline is illustrated in Figure~\ref{fig:mia_24}

% To explore cross-domain generalization, we investigate transfer learning. Models are first trained on MNIST and then fine-tuned on Fashion-MNIST by freezing convolutional layers and retraining the classifier. We evaluate whether temporal spike representations learned in one domain can retain both accuracy and privacy when transferred to a related task. Comparisons are drawn between training-from-scratch and transfer settings to quantify generalization gaps and privacy retention.



% Input images are resized to $32 \times 32$ and normalized; tabular features are scaled to [0, 1]. All models are implemented using the PyTorch-based \texttt{snnTorch} library, executed on GPU-enabled high-performance computing nodes. Image datasets are processed with a convolutional SNN (SNNConvNet), and tabular datasets use a fully connected SNN(SNNFCNet). All models run for 100 timesteps, using LIF neurons with $\beta = 0.95$, a batch size of 128, and Adam optimizer with a learning rate of 0.001.

\begin{table}[ht!]
\centering
\caption{Impact of temporal dynamics on accuracy and MIA AUC}
\label{tab:snn_mia_resilience}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{p{1.6cm} p{1.9cm} p{1.2cm} p{1cm} p{1.5cm}}
\toprule
\textbf{Dataset} & \textbf{Temporal Dynamics} & \textbf{Train Acc} & \textbf{Test Acc} & \textbf{Attack AUC} \\
\midrule
\multirow{3}{*}{\textbf{MNIST}}        
    & Rate              & 99.97\% & 99.26\% & \textbf{0.525(±0.010)} \\
    & Poisson\_Burst    & 99.89\% & 99.09\% & \textbf{0.519(±0.012)} \\
    & Delayed\_Burst    & 98.75\% & 98.04\% & \textbf{0.511(±0.019)} \\    
\midrule
\multirow{3}{*}{\textbf{F-MNIST}}      
    & Rate              & 99.06\% & 90.61\% & \textbf{0.543(±0.048)} \\
    & Poisson\_Burst    & 93.10\% & 88.99\% & \textbf{0.511(±0.012)} \\
    & Delayed\_Burst    & 91.89\% & 89.41\% & \textbf{0.511(±0.013)} \\ 
\midrule
\multirow{3}{*}{\textbf{CIFAR-10}}     
    & Rate              & 73.46\% & 64.85\% & \textbf{0.541(±0.016)} \\
    & Poisson\_Burst    & 65.04\% & 60.42\% & \textbf{0.512(±0.017)} \\
    & Delayed\_Burst    & 62.75\% & 60.27\% & \textbf{0.525(±0.016)} \\ 
\midrule
\multirow{3}{*}{\textbf{Iris}}         
    & Rate              & 97.04\% & 96.67\% & \textbf{0.549(±0.065)} \\
    & Poisson\_Burst    & 96.67\% & 93.33\% & \textbf{0.435(±0.056)} \\
    & Delayed\_Burst    & 93.33\% & 83.33\% & \textbf{0.468(±0.096)} \\ 
\midrule
\multirow{3}{*}{\textbf{Breast Cancer}} 
    & Rate              & 98.90\% & 96.49\% & \textbf{0.545(±0.003)} \\
    & Poisson\_Burst    & 98.24\% & 97.37\% & \textbf{0.531(±0.003)} \\
    & Delayed\_Burst    & 97.67\% & 97.37\% & \textbf{0.489(±0.017)} \\ 
\bottomrule
\end{tabular}
\end{table}


% \begin{table}[ht!]
% \centering
% \caption{Train and test accuracy across temporal dynamics for MNIST, FMNIST, CIFAR-10, Iris, and Breast Cancer datasets.}
% \label{tab:snn_accuracy_only}
% \renewcommand{\arraystretch}{1.1}
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{p{1.6cm} p{2.2cm} p{1.7cm} p{1.7cm}}
% \toprule
% \textbf{Dataset} & \textbf{Temporal Dynamics} & \textbf{Train Acc} & \textbf{Test Acc} \\
% \midrule
% \multirow{3}{*}{\textbf{MNIST}}        
%     & Rate              & 99.97\% & 99.26\% \\
%     & Burst\_poisson    & 99.89\% & 99.09\% \\
%     & Delayed\_burst    & 98.75\% & 98.04\% \\    
% \midrule
% \multirow{3}{*}{\textbf{F-MNIST}}      
%     & Rate              & 99.06\% & 90.61\% \\
%     & Burst\_poisson    & 93.10\% & 88.99\% \\
%     & Delayed\_burst    & 91.89\% & 89.41\% \\ 
% \midrule
% \multirow{3}{*}{\textbf{CIFAR-10}}     
%     & Rate              & 73.46\% & 64.85\% \\
%     & Burst\_poisson    & 65.04\% & 60.42\% \\
%     & Delayed\_burst    & 62.75\% & 60.27\% \\ 
% \midrule
% \multirow{3}{*}{\textbf{Iris}}         
%     & Rate              & 97.04\% & 96.67\% \\
%     & Burst\_poisson    & 96.67\% & 93.33\% \\
%     & Delayed\_burst    & 93.33\% & 83.33\% \\ 
% \midrule
% \multirow{3}{*}{\textbf{Breast Cancer}} 
%     & Rate              & 98.90\% & 96.49\% \\
%     & Burst\_poisson    & 98.24\% & 97.37\% \\
%     & Delayed\_burst    & 97.67\% & 97.37\% \\ 
% \bottomrule
% \end{tabular}
% \end{table}
 
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=.9\linewidth, height=0.55\linewidth]{Figure/en_accuracy_sum.pdf}
%     % \includegraphics[width=\linewidth]{Figure/mia_1sm.png}
%     \caption{Impact of different temporal dynamics on model performance across MNIST, Fashion-MNIST, CIFAR-10, Iris, and Breast Cancer datasets.} 
%     \label{fig:acc}
% \end{figure}

% \vspace{-1em}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=.9\linewidth, height=0.55\linewidth]{Figure/td_privacy_sum.pdf}
%     \caption{Impact of different temporal dynamics on privacy preservation across MNIST, Fashion-MNIST, CIFAR-10, Iris, and Breast Cancer datasets.}
%     \label{fig:priv}
% \end{figure}

Our experimental setup includes five datasets: MNIST, Fashion-MNIST, CIFAR-10 (image), and Iris and Breast Cancer (tabular). The results in  Table~\ref{tab:snn_mia_resilience} show a nuanced trade-off between model performance and privacy across temporal spike dynamics.  Poisson Burst and Delayed Burst transformations, inspired by cortical burst coding and sensory latency responses, consistently enhance privacy by lowering MIA attack AUC compared to the Rate baseline. For instance, Delayed Burst yields a 5–11\% reduction in AUC across all datasets, with the most notable privacy gains observed on Breast Cancer (0.545 to 0.489) and Iris (0.549 to 0.468). These patterns suggest that introducing temporal irregularity or onset latency can significantly degrade an attacker’s ability to distinguish training data from unseen samples. However, this privacy benefit often comes at a cost in classification performance. On CIFAR-10, both  Poisson Burst and Delayed Burst exhibit 4–7\% drops in test accuracy relative to the Rate baseline. On simpler datasets like MNIST and FMNIST, the performance degradation is more modest, typically staying under 1.5\%. Burst Poisson in particular demonstrates a strong privacy–utility balance, maintaining accuracy within 1–3\% of the baseline while achieving 2–5\% reductions in MIA vulnerability.




==> sections/misc.tex <==
As machine learning systems handle increasingly sensitive data, the potential for privacy violations grows. Li et al.    ~\cite{liu2021machine} categorize these privacy challenges into two primary areas: privacy attacks and privacy-preserving techniques. Privacy attacks have emerged as a critical concern in ML due to the growing realization that models can act as unintended leak vectors. These attacks can broadly be classified into different types, such as model inversion attacks, model extraction attacks, MIA. Model inversion attacks~\cite{fredrikson2015model} reconstruct input data from model outputs, while model extraction attacks ~\cite{juuti2019prada} aim to replicate a model’s functionality without direct access to its architecture or parameters. Among these, MIAs have gained significant attention due to their ability to infer whether a specific data point was used in training a model. According to the survey conducted by ~\cite{hu2022membership}, MIAs were first proposed in the context of genomic data by Homer et al.~\cite{homer2008resolving} where an attacker could infer if an individual's genome was part of a dataset based on summary statistics. Later, Shokri et al.\cite{shokri} introduced the first systematic MIA framework, showing how adversaries could use shadow models to infer training data membership. Salem et al. ~\cite{salem2018ml} reduced the complexity by demonstrating that a single shadow model can perform well compared to using multiple models, and they introduced metric-based attacks that rely on confidence scores and entropy without the need for identical data distribution between shadow and target models. Nasr et al.~\cite{nasr2019comprehensive} further expanded MIA into white-box settings, demonstrating that attackers with access to internal model parameters can perform even more effective MIAs. Melis et al.~\cite{melis2019exploiting} extended MIA to federated learning, showing vulnerabilities even in distributed learning settings, where multiple parties collaboratively train a model. Song and Mittal~\cite{song2021systematic} highlighted the increased privacy risks in generative models such as GANs, where membership inference attacks could be carried out on synthetic data generators. Recent work by Ilyas et al. introduced LiRA (Likelihood Ratio Attack) ~\cite{carlini2022membership}, a method that further improves the accuracy of MIAs by leveraging confidence scores more effectively to distinguish between training and non-training data points.In 2024, Zarifzadeh et al.~\cite{zarifzadeh2024low} introduced RMIA, a high-power membership inference attack that outperforms prior methods like LiRA and Attack-R, demonstrating superior robustness, particularly at low FPRs, using likelihood ratio tests.
While much of the data privacy research has centered around ANNs, expanding these investigations to SNNs is necessary. SNNs not only offer performance levels comparable to ANNs but also exhibit superior energy efficiency and hardware integration capabilities, positioning them as promising candidates for exploring inherent privacy features. Although privacy attacks on neuromorphic architectures remain underexplored, existing studies have yet to confirm SNNs' potential resistance to such threats. However, significant strides have been made in privacy-preserving techniques within the neuromorphic domain. For instance, recent efforts by Han et al. ~\cite{han2023towards} focus on developing privacy-preserving methods for SNNs, particularly utilizing FL and DP to address both computational efficiency and privacy challenges. Li et al.\cite{li2023efficient} introduced a framework that combines Fully Homomorphic Encryption (FHE) with SNNs, enabling encrypted inference while preserving SNNs' energy efficiency and computational advantages. Similarly, Nikfam et al.\cite{nikfam2023homomorphic} developed an HE framework tailored for SNNs, offering enhanced accuracy over DNNs under encryption, while carefully balancing computational efficiency. Additionally, Safronov et al.\cite{kim2022privatesnn} proposed PrivateSNN, a privacy-preserving framework for SNNs that employs differential privacy to mitigate membership inference attacks, maintaining the energy-efficient nature of SNNs.


The escalating computational demands of deep neural networks (DNNs), characterized by increased parameter counts and complex operations, have propelled quantization as a leading approach for reducing model size and computational load. Quantization compresses neural networks by reducing the precision of parameters, such as weights and activations, which lowers the memory footprint and enables efficient deployment on resource-constrained devices without substantial performance loss \cite{yang2019quantization, nagel2021white}. Early work on quantization focused on inference, using methods such as post-training quantization (PTQ) and quantization-aware training (QAT), which apply low-bit representations across entire network layers \cite{jacob2018quantization}. Recent advancements, like adaptive quantization frameworks, have further enhanced efficiency by dynamically adjusting bit-widths per layer, achieving higher compression rates while preserving accuracy \cite{tran2024privacy, zhou2021balanced}.

Quantization has emerged not only as an efficiency tool but also as a subtle defense mechanism in privacy-sensitive applications. This line of inquiry is particularly important given the vulnerability of DNNs to membership inference attacks (MIA), where adversaries exploit model confidence to infer whether specific data was part of the training set \cite{kowalski2022towards}. Quantized models, by introducing noise and reducing overfitting, have shown inherent resilience against such attacks, suggesting a potential dual role for quantization in enhancing privacy \cite{famili2023deep}. Experimental results have demonstrated that quantized models yield lower precision in MIA success rates compared to full-precision models, reducing the adversary’s ability to extract sensitive information without compromising model accuracy \cite{wei2024q, hu2021quantized}.

In recent years, these quantization techniques have been adapted for Spiking Neural Networks (SNNs), a neuromorphic approach inspired by biological neurons, which operate efficiently in edge computing environments due to their low energy consumption and sparse activity patterns. The development of quantization frameworks tailored to SNNs, such as Q-SpiNN and QFFS, has addressed unique challenges in quantizing synaptic weights, membrane potentials, and spike dynamics, crucial for maintaining the model’s accuracy and efficiency on low-power devices \cite{putra2021q, li2022quantization}. These frameworks use methods like integer quantization and fixed-point representation to optimize computational loads while preserving the distinctive temporal dynamics of SNNs, thus achieving a balance between efficiency and accuracy in neuromorphic hardware.

The privacy implications of quantized SNNs, however, remain an under-explored frontier. Given the inherent sparsity and quantized nature of SNNs, these networks hold promise for robust privacy preservation against attacks like MIA. By constraining information representation and introducing noise, quantized SNNs may naturally reduce the leakage pathways adversaries exploit. This potential resilience provides strong motivation for further investigation into quantized SNNs as a privacy-preserving framework, paving the way for more secure neuromorphic models in sensitive applications. This work aims to build on these foundational insights, exploring the intersection of quantization, efficiency, and privacy within SNNs \cite{schaefer2020quantizing, stock2019and, kowalski2022towards}.



% \begin{figure*}[ht]
%     \centering
    
%     % First row - MNIST and F-MNIST
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/ann_mnist_acc.png}
%         \caption*{ANN}
%         \label{fig:mnist_ann}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/snn_mnist_acc.png}
%         \caption*{SNN}
%         \label{fig:mnist_snn}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/ann_fmnist_acc.png}
%         \caption*{ANN}
%         \label{fig:fmnist_ann}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/snn_fmnist_acc.png}
%         \caption*{SNN}
%         \label{fig:fmnist_snn}
%     \end{subfigure}
%     \caption*{(a) MNIST \hspace{8cm} (b) F-MNIST}
    
%     % Second row - CIFAR-10 and CIFAR-100
%     \vspace{1em}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/ann_cifar10_acc.png}
%         \caption*{ANN}
%         \label{fig:cifar10_ann}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/snn_cifar10_acc.png}
%         \caption*{SNN}
%         \label{fig:cifar10_snn}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/ann_bc_acc.png}
%         \caption*{ANN}
%         \label{fig:cifar100_ann}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/snn_bc_acc.png}
%         \caption*{SNN}
%         \label{fig:cifar100_snn}
%     \end{subfigure}
%     \caption*{(c) CIFAR-10 \hspace{8cm} (d) Breast Cancer}
    
%     % Final caption for the entire figure
%     \caption{Activation Quantization impact on Model Accuracy in (a) MNIST, (b) F-MNIST, (c) CIFAR-10, and (d) Breast Cancer.}
%     \label{fig:act_acc}
% \end{figure*}


% \begin{figure*}[ht]
%     \centering
    
%     % First row - MNIST and F-MNIST
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/ann_mnist_auc.png}
%         \caption*{ANN}
%         \label{fig:mnist_ann}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/snn_mnist_auc.png}
%         \caption*{SNN}
%         \label{fig:mnist_snn}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/ann_fmnist_auc.png}
%         \caption*{ANN}
%         \label{fig:fmnist_ann}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/snn_fmnist_auc.png}
%         \caption*{SNN}
%         \label{fig:fmnist_snn}
%     \end{subfigure}
%     \caption*{(a) MNIST \hspace{8cm} (b) F-MNIST}
    
%     % Second row - CIFAR-10 and CIFAR-100
%     \vspace{1em}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/ann_cifar10_auc.png}
%         \caption*{ANN}
%         \label{fig:cifar10_ann}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/snn_cifar10_auc.png}
%         \caption*{SNN}
%         \label{fig:cifar10_snn}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/ann_bc_auc.png}
%         \caption*{ANN}
%         \label{fig:cifar100_ann}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/activation/snn_bc_auc.png}
%         \caption*{SNN}
%         \label{fig:cifar100_snn}
%     \end{subfigure}
%     \caption*{(c) CIFAR-10 \hspace{8cm} (d) Breast Cancer}
    
%     % Final caption for the entire figure
%     \caption{Activation Quantization impact on MIA AUC score in (a) MNIST, (b) F-MNIST, (c) CIFAR-10, and (d) Breast Cancer.}
%     \label{fig:act_acc}
% \end{figure*}



% \begin{figure*}[ht!]
%   \centering
%   % First row - MNIST and F-MNIST
%   \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/weight/ann_mnist_w_quant.png}
%     \caption*{ANN}
%     \label{fig:mnist_ann}
%   \end{subfigure}%
%   \hfill
%   \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/weight/snn_mnist_w_quant.png}
%     \caption*{SNN}
%     \label{fig:mnist_snn}
%   \end{subfigure}%
%   \hfill
%   \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/weight/ann_fmnist_w_quant.png}
%     \caption*{ANN}
%     \label{fig:fmnist_ann}
%   \end{subfigure}%
%   \hfill
%   \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/weight/snn_fmnist_w_quant.png}
%     \caption*{SNN}
%     \label{fig:fmnist_snn}
%   \end{subfigure}%
%   \caption*{(a) MNIST \hspace{8cm} (b) F-MNIST}
  
%   % Second row - CIFAR-10 and Iris
%   \vspace{1em}
%   \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/weight/ann_cifar10_w_quant.png}
%     \caption*{ANN}
%     \label{fig:cifar10_ann}
%   \end{subfigure}%
%   \hfill
%   \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/weight/snn_cifar10_w_quant.png}
%     \caption*{SNN}
%     \label{fig:cifar10_snn}
%   \end{subfigure}%
%   \hfill
%   \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/weight/ann_iris_w_quant.png}
%     \caption*{ANN}
%     \label{fig:iris_ann}
%   \end{subfigure}%
%   \hfill
%   \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/weight/snn_iris_w_quant.png}
%     \caption*{SNN}
%     \label{fig:iris_snn}
%   \end{subfigure}%
%   \caption*{(c) CIFAR-10 \hspace{8cm} (d) Iris}

%   % Third row - Breast Cancer only, centered
%   \vspace{1em}
%   \hspace{\fill} % Centering space
%   \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/weight/ann_bc_w_quant.png}
%     \caption*{ANN}
%     \label{fig:bc_ann}
%   \end{subfigure}%
%   \hspace{0.5cm} 
%   \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/weight/snn_bc_w_quant.png}
%     \caption*{SNN}
%     \label{fig:bc_snn}
%   \end{subfigure}%
%   \hspace{\fill} % Centering space
%   \caption*{(e) Breast Cancer}

%   % Final caption for the entire figure
%   \caption{Impact of weight quantization on ANN and SNN models across different datasets: (a) MNIST, (b) F-MNIST, (c) CIFAR-10, (d) Iris, and (e) Breast Cancer.}
%   \label{fig:dp_mia}
% \end{figure*}
